A Convex Method of Generalized State Estimation using Circuit-theoretic Node-breaker Model

An accurate and up-to-date topology is critical for situational awareness of a power grid; however, wrong switch statuses due to physical damage, communication error, or cyber-attack, can often result in topology errors. To maintain situation awareness under the possible topology errors and bad data, this paper develops ckt-GSE, a circuit-theoretic generalized state estimation method using node-breaker (NB) model. Ckt- GSE is a convex and scalable model that jointly estimates AC state variables and network topology, with robustness against different data errors. The method first constructs an equivalent circuit representation of the AC power grid by developing and aggregating linear circuit models of SCADA meters, phasor measurement units(PMUs), and switching devices. Then based on this circuit, ckt-GSE defines a constrained optimization problem using weighted least absolute value (WLAV) objective to form a robust estimator. The problem is a Linear Programming (LP) problem whose solution includes accurate AC states and a sparse vector of noise terms to identify topology errors and bad data.This paper is the first to explore a circuit-theoretic approach for an AC-network constrained GSE algorithm that is: 1) applicable to the real-world data setting, 2) convex without relaxation, scalable with our circuit-based solver; and 3) robust with the ability to identify and reject different data errors

==> article_abstract.tex <==

\section{Abstract}

Today’s grid operators rely on the situational awareness from AC state estimation (SE) algorithm.  Most current ACSE algorithms use bus-branch model that assume access to accurate network topology. Therefore, if assumed network topology is erroneous, the quality of SE solution will be adversely impacted. Further, topology error itself will not be detected by standard residual-based bad data detection (BDD) techniques. To readily access latest grid topology, network topology processor (NTP) is used in grid control rooms. NTP continuously processes the SCADA data for circuit breaker and switch status, and it feeds the network connectivity information into the bus-branch model used by ACSE. However, NTP algorithms in control room today do not account for wrong switch status data caused by communication errors, physical damages or cyber-attacks.

To tackle the problem of topological errors, many methods have been proposed\cite{TE-GSE}\cite{TE-WLSE-BDI}\cite{TESE-GSE-PMUabur}\cite{convexTESE-SDP-weng}. Generalized topology processing \cite{TE-GSE}, also known as generalized state estimation, creates pseudo-measurements for switches and applies hypothesis tests to detect wrong switching status. Similarly, a variant of standard SE BDD \cite{TE-WLSE-BDI} handles wrong status data by spawning SE with different possible topologies and assuming that the optimal topology gives the smallest residual. More recently, other advanced methods have been developed where TE and ACSE are merged together into a node-breaker (NB) model to perform generalized state estimation\cite{TESE-GSE-PMUabur}\cite{convexTESE-SDP-weng}. This allows combined identification and localization of both bad analog data and wrong status data. However, all these methods have significant drawbacks prohibiting them to be of practical value.

For instance, generalized topology processing\cite{TE-GSE} was shown to run on a DC grid model of a small sub-network in the vicinity of suspected errors, which results in significant loss of solution accuracy. When extended to AC model with non-linear remote terminal unit (RTU) models, the problem becomes non-convex and hard to solve. Alternatively, the method to fix erroneous topology from SE residual tests\cite{TE-WLSE-BDI}, apart from being non-convex, faces rapid growth of burden under conditions of multiple wrong switch status where finding the optimal topology becomes a combinatorial optimization problem and computationally intractable. While some advanced NB model based methods \cite{TESE-GSE-PMUabur}, \cite{convexTESE-SDP-weng} provide a convex formulations for generalized state estimation; their application is \cite{TESE-GSE-PMUabur} either limited to systems with only PMU measurements or is based on convex relaxations (e.g. semi-definite programming methods in \cite{convexTESE-SDP-weng}) that do not scale well to large-scale problems.

To address the challenges described above, this paper proposes  a generalized state estimation algorithm from a circuit-theoretic viewpoint, using NB model. We will show that the algorithm is robust against wrong status data and bad-measurements while being computationally tractable and scalable to large practical networks. 
%In this approach we will represent the electrical grid using a node-breaker model that will be mapped into an equivalent circuit. 
We will build novel circuit models for open/closed switching devices, which together with previously developed analog measurement models\cite{sugar-se-L2} will replace the measured grid components with linear circuit elements and map the original system into a linear circuit. To consider bad analog measurement data and wrong status/topology data, we will add noise terms to these circuit models. Then a robust generalized state estimation of the network can be formulated by minimizing least absolute (LAV) value of the noise terms in circuit models. Due to linear network constraints, the problem will be formulated as a Linear Programming (LP) problem with provably guaranteed convergence. Meanwhile, the algorithm will produce a sparse vector of noise terms that allows localization of spurious analog measurement or switch status. The proposed method of generalized state estimation provides the benefit of 1) convexity 2) intrinsic robustness against bad analog measurement and topological errors.



